Kappa-Minkowski spacetime: mathematical formalism and applications in Planck scale physics

The dissertation presents possibilities of applying noncommutative spacetimes description, particularly kappa-deformed Minkowski spacetime and Drinfeld's deformation theory, as a mathematical formalism for Doubly Special Relativity theories (DSR), which are thought as phenomenological limit of quantum gravity theory. Deformed relativistic symmetries are described within Hopf algebra language. In the case of (quantum) kappa-Minkowski spacetime the symmetry group is described by the (quantum) kappa-Poincare Hopf algebra. Deformed relativistic symmetries were used to construct the DSR algebra, which unifies noncommutative coordinates with generators of the symmetry algebra. It contains the deformed Heisenberg-Weyl subalgebra. It was proved that DSR algebra can be obtained by nonlinear change of generators from undeformed algebra. We show that the possibility of applications in Planck scale physics is connected with certain realizations of quantum spacetime, which in turn leads to deformed dispersion relations.

==> part3.tex <==

\newpage
 \thispagestyle{empty}
\vspace{2cm}


\begin{center}
    {\LARGE PART III}
\end{center}

\vspace{1.5cm}
\begin{center}
    
\textsc{ \Huge Curriculum {Vitae}\\
and}
\textsc{ \Huge  Publications}

\end{center}
\vspace{9.0cm}
%\hspace{\stretch{1}} \begin{flushright}
%     \emph{"Mathematics may be defined as the subject\\ in which we never know what we are talking about,\\ nor whether what we are saying is true."}
%\end{flushright}
%\begin{flushright}
%    Bertrand Russell 
%\end{flushright}
%
%\vspace{1.0cm}
%\hspace{\stretch{1}} \begin{flushright}
%     \emph{"As far as the laws of mathematics refer to reality,\\ they are not certain, and as far as they are certain,\\ they do not refer to reality."}
%\end{flushright}
%   \begin{flushright}
%     Albert Einstein
%\end{flushright}
%
%
%
%\vspace{5.0cm}


\newpage
\thispagestyle{empty}


